Mixture of Weak & Strong Experts on Graphs

Realistic graphs contain both (1) rich self-features of nodes and (2) informative structures of neighborhoods, jointly handled by a Graph Neural Network (GNN) in the typical setup. We propose to decouple the two modalities by Mixture of weak and strong experts (Mowst), where the weak expert is a light-weight Multi-layer Perceptron (MLP), and the strong expert is an off-the-shelf GNN. To adapt the experts' collaboration to different target nodes, we propose a "confidence" mechanism based on the dispersion of the weak expert's prediction logits. The strong expert is conditionally activated in the low-confidence region when either the node's classification relies on neighborhood information, or the weak expert has low model quality. We reveal interesting training dynamics by analyzing the influence of the confidence function on loss: our training algorithm encourages the specialization of each expert by effectively generating soft splitting of the graph. In addition, our "confidence" design imposes a desirable bias toward the strong expert to benefit from GNN's better generalization capability. Mowst is easy to optimize and achieves strong expressive power, with a computation cost comparable to a single GNN. Empirically, Mowst on 4 backbone GNN architectures show significant accuracy improvement on 6 standard node classification benchmarks, including both homophilous and heterophilous graphs (https://github.com/facebookresearch/mowst-gnn).

==> figures/fig_denoise.tex <==
\begin{wrapfigure}{r}{0.33\textwidth} 
 \centering
 \includegraphics[width=0.33\textwidth]{figures/flickr_tsne0_20.pdf}
  \caption{\flickr: The t-SNE representations demonstrate the denoised fine-tuning process of {\moe}.}\label{fig:denoise}
\end{wrapfigure}

==> figures/fig_mowst_diagram.tex <==
\begin{figure}[h]
    \centering
    \begin{subfigure}{0.31\linewidth}
        \centering
        \includegraphics[width=0.9\textwidth]{figures/mowst_inference_cropped.pdf}
        \caption{{\moe} inference.}
        \label{fig:diagram_mowst_inference}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.68\linewidth}
        \centering
        \includegraphics[width=0.9\textwidth]{figures/mowst_training_cropped.pdf}
        \caption{{\moe} training.}
        \label{fig:diagram_mowst_training}
    \end{subfigure}
    \caption{\camera{The diagram of the inference and training algorithms of \moe.}}
    \label{fig:mowst_diagram}
\end{figure}



==> plots/illustration_C_bound.tex <==
\begin{tikzpicture}
\begin{axis}[
    xlabel={$p$},
    ylabel={$y$},
    domain=0:1, % Specify the domain of the function
    ymin=0,
    ymax=2,
    xmin=0,
    xmax=1,
    samples=500,  % Number of points to sample
    axis lines=middle, % Draw the axis in the middle
    grid, % Add a grid
    legend style={at={(0.5,-0.2)},anchor=north},
]
\def\alphaVal{0.7}
\def\muVal{0.9}

\addplot[blue,thick] {-\alphaVal * ln(x) - (1-\alphaVal) * ln(1-x)}; 

\pgfmathsetmacro\yDelta{-\alphaVal*ln(\alphaVal) - (1-\alphaVal) * ln(1-\alphaVal)}
\pgfmathsetmacro\yMu{-\alphaVal*ln(\muVal) - (1-\alphaVal) * ln(1-\muVal)}
\addplot[scatter,only marks,mark=*,mark size=3pt,mark options={fill=red}] coordinates{(\alphaVal, \yDelta)} node[above] {$\Delta\paren{\bm{\alpha}}$};

\addplot[scatter,only marks,mark=*,mark size=3pt,mark options={fill=red}] coordinates{(1-\alphaVal, \yDelta)} node[above] {};

\addplot[scatter,only marks,mark=*,mark size=3pt,mark options={fill=red}] coordinates{(\muVal, \yMu)} node[below] {};

\draw[dotted] (0, \yMu) -- (\muVal, \yMu);

\draw (0,0) -- (1,1);

\legend{$\sin(x)$}
\end{axis}
\end{tikzpicture}

==> tables/comp_gin.tex <==
\begin{tabular}{lccccc}
\toprule[1.1pt]
                            & \flickr        & \arxiv    & \penn       & \pokec        & \twitch \\
                            \midrule
GCN                         & 53.86 \small{$\textcolor{gray}{\pm 0.37}$} &  71.74$^{\dagger}$ \small{$\textcolor{gray}{\pm 0.29}$} & 82.17 \small{$\textcolor{gray}{\pm 0.04}$} & 76.01 \small{$\textcolor{gray}{\pm 0.49}$} & 62.42 \small{$\textcolor{gray}{\pm 0.53}$} \\
\multirow{2}{*}{\moebothgnn{GCN}}  & 54.62 \small{$\textcolor{gray}{\pm 0.23}$} & \textbf{72.52} \small{$\textcolor{gray}{\pm 0.07}$} & 83.19 \small{$\textcolor{gray}{\pm 0.43}$} & 77.28 \small{$\textcolor{gray}{\pm 0.08}$} & 63.74 \small{$\textcolor{gray}{\pm 0.23}$} \\
& (\greentext{\textbf{+0.76}})        & (\greentext{\textbf{+0.78}})        & (\greentext{\textbf{+1.02}})        & (\greentext{\textbf{+1.27}})          \\
GCN-skip                         & 52.98 \small{$\textcolor{gray}{\pm 0.00}$} &  69.56 \small{$\textcolor{gray}{\pm 0.00}$} & 76.58 \small{$\textcolor{gray}{\pm 0.53}$} & 73.46 \small{$\textcolor{gray}{\pm 0.04}$} & 61.05 \small{$\textcolor{gray}{\pm 0.23}$} \\
                            \midrule
GIN                         & 53.71 \small{$\textcolor{gray}{\pm 0.35}$} &   69.39   \small{$\textcolor{gray}{\pm 0.56}$}         & 82.68 \small{$\textcolor{gray}{\pm 0.32}$} & 53.37 \small{$\textcolor{gray}{\pm 2.15}$} & 61.76 \small{$\textcolor{gray}{\pm 0.60}$} \\
\multirow{2}{*}{\moebothgnn{GIN}}                        & \textbf{55.48} \small{$\textcolor{gray}{\pm 0.32}$} &  71.43 \small{$\textcolor{gray}{\pm 0.26}$} & \textbf{84.56} \small{$\textcolor{gray}{\pm 0.31}$} & 76.11 \small{$\textcolor{gray}{\pm 0.39}$} & 64.32 \small{$\textcolor{gray}{\pm 0.34}$} \\
& (\greentext{\textbf{+1.77}})        & (\greentext{\textbf{+2.04}})        & (\greentext{\textbf{+1.88}})        & (\greentext{\textbf{+22.74}})        & (\greentext{\textbf{+2.56}})        \\
GIN-skip                         & 52.70 \small{$\textcolor{gray}{\pm 0.00}$} &  71.28 \small{$\textcolor{gray}{\pm 0.00}$} & 80.32 \small{$\textcolor{gray}{\pm 0.43}$} & 76.29 \small{$\textcolor{gray}{\pm 0.51}$} & 64.27 \small{$\textcolor{gray}{\pm 0.25}$} \\
\multirow{2}{*}{\moebothgnn{GIN-skip}}                         & 53.19 \small{$\textcolor{gray}{\pm 0.31}$} &  71.79 \small{$\textcolor{gray}{\pm 0.23}$} & 81.20 \small{$\textcolor{gray}{\pm 0.55}$} & \textbf{79.70} \small{$\textcolor{gray}{\pm 0.23}$} & \textbf{64.91} \small{$\textcolor{gray}{\pm 0.22}$} \\
& (\greentext{\textbf{+0.49}})        & (\greentext{\textbf{+0.51}})        & (\greentext{\textbf{+0.88}})        & (\greentext{\textbf{+3.41}})        & (\greentext{\textbf{+0.64}})        \\
                            \bottomrule[1.1pt]
\end{tabular}

==> tables/full_comp_gin.tex <==
\begin{table}[h]
    \centering
    \caption{{\moe} consistently improves the GIN baseline and its variants with skip connection.}
    \label{tab:main_comp_gin_res}
    % \scriptsize
    % \vspace{-5pt}
    \adjustbox{max width=\textwidth}{
\begin{tabular}{lcccccr}
\toprule[1.1pt]
                            & \flickr        & \arxiv    & \penn       & \pokec        & \twitch & Average gain\\
                            \midrule
GCN                         & 53.86 \small{$\textcolor{gray}{\pm 0.37}$} &  71.74 \small{$\textcolor{gray}{\pm 0.29}$} & 82.17 \small{$\textcolor{gray}{\pm 0.04}$} & 76.01 \small{$\textcolor{gray}{\pm 0.49}$} & 62.42 \small{$\textcolor{gray}{\pm 0.53}$} & -\\
\multirow{2}{*}{\moebothgnn{GCN}}  & 54.62 \small{$\textcolor{gray}{\pm 0.23}$} & \textbf{72.52} \small{$\textcolor{gray}{\pm 0.07}$} & 83.19 \small{$\textcolor{gray}{\pm 0.43}$} & 77.28 \small{$\textcolor{gray}{\pm 0.08}$} & 63.74 \small{$\textcolor{gray}{\pm 0.23}$} & \multirow{2}{*}{\greentext{\textbf{1.03}}}\\
& \small{(\greentext{\textbf{+0.76}})}        & \small{(\greentext{\textbf{+0.78}})}        & \small{(\greentext{\textbf{+1.02}})}        & \small{(\greentext{\textbf{+1.27}})}        & \small{(\greentext{\textbf{+1.32}})}        \\
GCN-skip                         & 52.98 \small{$\textcolor{gray}{\pm 0.00}$} &  69.56 \small{$\textcolor{gray}{\pm 0.00}$} & 76.58 \small{$\textcolor{gray}{\pm 0.53}$} & 73.46 \small{$\textcolor{gray}{\pm 0.04}$} & 61.05 \small{$\textcolor{gray}{\pm 0.23}$} & - \\
                            \midrule
GIN                         & 53.71 \small{$\textcolor{gray}{\pm 0.35}$} &   69.39   \small{$\textcolor{gray}{\pm 0.56}$}         & 82.68 \small{$\textcolor{gray}{\pm 0.32}$} & 53.37 \small{$\textcolor{gray}{\pm 2.15}$} & 61.76 \small{$\textcolor{gray}{\pm 0.60}$} & -\\
\multirow{2}{*}{\moebothgnn{GIN}}                        & \textbf{55.48} \small{$\textcolor{gray}{\pm 0.32}$} &  71.43 \small{$\textcolor{gray}{\pm 0.26}$} & \textbf{84.56} \small{$\textcolor{gray}{\pm 0.31}$} & 76.11 \small{$\textcolor{gray}{\pm 0.39}$} & 64.32 \small{$\textcolor{gray}{\pm 0.34}$} & \multirow{2}{*}{\greentext{\textbf{6.20}}}\\
& \small{(\greentext{\textbf{+1.77}})}        & \small{(\greentext{\textbf{+2.04}})}        & \small{(\greentext{\textbf{+1.88}})}        & \small{(\greentext{\textbf{+22.74}})}        & \small{(\greentext{\textbf{+2.56}})}        \\
GIN-skip                         & 52.70 \small{$\textcolor{gray}{\pm 0.00}$} &  71.28 \small{$\textcolor{gray}{\pm 0.00}$} & 80.32 \small{$\textcolor{gray}{\pm 0.43}$} & 76.29 \small{$\textcolor{gray}{\pm 0.51}$} & 64.27 \small{$\textcolor{gray}{\pm 0.25}$} & -\\
\multirow{2}{*}{\moebothgnn{GIN-skip}}                         & 53.19 \small{$\textcolor{gray}{\pm 0.31}$} &  71.79 \small{$\textcolor{gray}{\pm 0.23}$} & 81.20 \small{$\textcolor{gray}{\pm 0.55}$} & \textbf{79.70} \small{$\textcolor{gray}{\pm 0.23}$} & \textbf{64.91} \small{$\textcolor{gray}{\pm 0.22}$} & \multirow{2}{*}{\greentext{\textbf{1.19}}}\\
& \small{(\greentext{\textbf{+0.49}})}        & \small{(\greentext{\textbf{+0.51}})}        & \small{(\greentext{\textbf{+0.88}})}        & \small{(\greentext{\textbf{+3.41}})}        & \small{(\greentext{\textbf{+0.64}})}        \\
                            \bottomrule[1.1pt]
\end{tabular}}
\end{table}

